Diffusion Priors for Dynamic View Synthesis from Monocular Videos

Dynamic novel view synthesis aims to capture the temporal evolution of visual content within videos. Existing methods struggle to distinguishing between motion and structure, particularly in scenarios where camera poses are either unknown or constrained compared to object motion. Furthermore, with information solely from reference images, it is extremely challenging to hallucinate unseen regions that are occluded or partially observed in the given videos. To address these issues, we first finetune a pretrained RGB-D diffusion model on the video frames using a customization technique. Subsequently, we distill the knowledge from the finetuned model to a 4D representations encompassing both dynamic and static Neural Radiance Fields (NeRF) components. The proposed pipeline achieves geometric consistency while preserving the scene identity. We perform thorough experiments to evaluate the efficacy of the proposed method qualitatively and quantitatively. Our results demonstrate the robustness and utility of our approach in challenging cases, further advancing dynamic novel view synthesis.

==> figures/pipeline.tex <==
\begin{figure*}[tbh]
\centering
\includegraphics[width=1.0\textwidth, clip]{figures/framework.pdf}
\caption{\textbf{AToM pipeline.} AToM optimizes a feed-forward Text-to-Mesh generator, which consists of three components: a text encoder that tokenizes the input prompt, a text-to-tiplane network that outputs a triplane representation from the text embedding, and a 3D network that generates a differential mesh directly through SDF, deformation, and texture modules from triplane features and queried positions and their positional embedding. 
During training, AToM utilizes a two-stage mechanism, where the first stage leverages stable but expensive volumetric optimization to train only the SDF and textures modules using low-resolution renderings, and the seconds stage uses mesh rasterization to optimize the whole network through high-resolution renderings to yield high-quality 3D content.
AToM is optimized on many prompts simultaneously through the guidance of a text-to-image diffusion prior without 3D data supervision in both stages.
}
\label{fig:pipeline}
\end{figure*}

==> figures/teaser.tex <==

% \begin{figure*}[H]
% \centering
% \includegraphics[page=3,width=1.0\textwidth, trim= 0 9.5cm 12cm 0, clip]{figures/src/pipeline.pdf}
% \caption{\textbf{Comparisons against DreamFusion \cite{DreamFusion}, ATT3D \cite{ATT3D}, and our AToM.} 
% DreamFusion optimizes a per-prompt Neural Radiance Field (NeRF), requiring around 2 hours to render a single 3D model. ATT3D amortizes the training, generates 3D content in seconds during inference, but still requires expensive marching cube to produce a textued mesh. 
% Our AToM optimizes a feed-forward Text-to-Mesh generator that offers  meshes in 2 second with better quality and higher CLIP-Similarity. 
% }
% \label{fig:teaser}
% \end{figure*}


% \newcommand\myfigure{%
%   \makebox[0pt]{\hspace{17.5cm}\includegraphics[page=3,width=1.0\textwidth, trim= 0 9.5cm 12cm 0, clip]{figures/teaser.pdf}}
%   \\
%   \refstepcounter{figure}\normalfont{Figure~\thefigure: \textbf{Novel view synthesis from monocular videos.} 
% TEASER }
%   \label{fig:teaser}
% }

\newcommand\myfigure{%
  \makebox[0pt]{\hspace{17.5cm}\includegraphics[page=3,width=1.0\textwidth, trim= 0 9.5cm 12cm 0, clip]{figures/teaser.pdf}}
  \\
  \refstepcounter{figure}\normalfont{Figure~\thefigure: \textbf{Novel view synthesis from monocular videos.} 
TEASER }
  \label{fig:teaser}
}



==> figures/triplane.tex <==
\begin{figure}[tbh]
\centering
\includegraphics[page=2,width=1.0\columnwidth, trim= 0 14.7cm 21cm 0, clip]{figures/src/pipeline.pdf}
\caption{\textbf{Text-to-Triplane architecture.} Triplane is generated from the token-averaged text embedding by a linear projection and a reshaping operator and is refined through the proposed text-conditioned 3D-aware ConvNeXt network.}
\label{fig:triplane}
\end{figure}

==> new_pipeline.tex <==
%% Creator: Inkscape 1.2.1 (9c6d41e, 2022-07-14), www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'g4554.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \newcommand*\fsize{\dimexpr\f@size pt\relax}%
  \newcommand*\lineheight[1]{\fontsize{\fsize}{#1\fsize}\selectfont}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{585.08868408bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.30454699)%
    \lineheight{1}%
    \setlength\tabcolsep{0pt}%
    \put(0,0){\includegraphics[width=\unitlength,page=1]{g4554.pdf}}%
    \put(0.82167991,0.28622289){\color[rgb]{0,0,0}\makebox(0,0)[t]{\lineheight{1.25}\smash{\begin{tabular}[t]{c}4D representation \end{tabular}}}}%
    \put(0.7782667,0.1338362){\color[rgb]{0,0,0}\makebox(0,0)[t]{\lineheight{1.25}\smash{\begin{tabular}[t]{c}Blend\end{tabular}}}}%
    \put(0.8186114,0.13271455){\color[rgb]{0,0,0}\makebox(0,0)[t]{\lineheight{1.25}\smash{\begin{tabular}[t]{c}\textit{⨁}\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=2]{g4554.pdf}}%
    \put(0.25829378,0.28697395){\color[rgb]{0,0,0}\makebox(0,0)[t]{\lineheight{1.25}\smash{\begin{tabular}[t]{c}Casual Input Video with Monocular Depth \end{tabular}}}}%
    \put(0.24845758,0.11365037){\color[rgb]{0,0,0}\makebox(0,0)[t]{\lineheight{1.25}\smash{\begin{tabular}[t]{c}LDM3D Diffusion \end{tabular}}}}%
    \put(0.24686799,0.02067676){\color[rgb]{0,0,0}\makebox(0,0)[t]{\lineheight{1.25}\smash{\begin{tabular}[t]{c}\textit{"a young boy sitting on a large piece of furniture"} \end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=3]{g4554.pdf}}%
    \put(0.2478945,0.14700706){\color[rgb]{0,0,0}\makebox(0,0)[t]{\lineheight{1.25}\smash{\begin{tabular}[t]{c}DreamBooth fine-tuning \end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=4]{g4554.pdf}}%
    \put(0.2496306,0.07190671){\color[rgb]{0,0,0}\makebox(0,0)[t]{\lineheight{1.25}\smash{\begin{tabular}[t]{c}U-Net \end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=5]{g4554.pdf}}%
    \put(0.82053419,0.07675014){\color[rgb]{0,0,0}\makebox(0,0)[t]{\lineheight{1.25}\smash{\begin{tabular}[t]{c}Static NeRF \end{tabular}}}}%
    \put(0.81420565,0.03236496){\color[rgb]{0,0,0}\makebox(0,0)[t]{\lineheight{1.25}\smash{\begin{tabular}[t]{c}\textit{XYZ} \end{tabular}}}}%
    \put(0.82099988,0.24167057){\color[rgb]{0,0,0}\makebox(0,0)[t]{\lineheight{1.25}\smash{\begin{tabular}[t]{c}Dynamic NeRF \end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=6]{g4554.pdf}}%
    \put(0.77804652,0.19874585){\color[rgb]{0,0,0}\makebox(0,0)[t]{\lineheight{1.25}\smash{\begin{tabular}[t]{c}\textit{XYT} \end{tabular}}}}%
    \put(0.8135745,0.19872643){\color[rgb]{0,0,0}\makebox(0,0)[t]{\lineheight{1.25}\smash{\begin{tabular}[t]{c}\textit{YZT} \end{tabular}}}}%
    \put(0.84939514,0.19914566){\color[rgb]{0,0,0}\makebox(0,0)[t]{\lineheight{1.25}\smash{\begin{tabular}[t]{c}\textit{XZT} \end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=7]{g4554.pdf}}%
    \put(0.96619574,0.23920757){\color[rgb]{0,0,0}\makebox(0,0)[t]{\lineheight{0.5}\smash{\begin{tabular}[t]{c}Input\\Camera \end{tabular}}}}%
    \put(0.96610895,0.17007889){\color[rgb]{0,0,0}\makebox(0,0)[t]{\lineheight{0.5}\smash{\begin{tabular}[t]{c}Input\\Timestamp \end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=8]{g4554.pdf}}%
    \put(0.96619572,0.09229976){\color[rgb]{0,0,0}\makebox(0,0)[t]{\lineheight{0.5}\smash{\begin{tabular}[t]{c}Random\\Camera \end{tabular}}}}%
    \put(0.96610892,0.02317109){\color[rgb]{0,0,0}\makebox(0,0)[t]{\lineheight{0.5}\smash{\begin{tabular}[t]{c}Random\\Timestamp \end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=9]{g4554.pdf}}%
    \put(0.64509879,0.01213239){\color[rgb]{0,0,0}\makebox(0,0)[t]{\lineheight{0.80000001}\smash{\begin{tabular}[t]{c}Random viewpoint rendering \end{tabular}}}}%
    \put(0.64504538,0.16209697){\color[rgb]{0,0,0}\makebox(0,0)[t]{\lineheight{0.80000001}\smash{\begin{tabular}[t]{c}Input viewpoint rendering \end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=10]{figures/new_pipeline.pdf}}%
  \end{picture}%
\endgroup%


==> sections/intro.tex <==
\section{Introduction}

Motivation:
\begin{itemize}
    \item Reconstructing dynamic scene is an ill-posed problem (compared to static scene reconstruction) and challenging to solve. Prior methods attempt to approach this problem either through hand-crafted geometric and physics priors (cite Nerfies, HyperNeRF) or leverage monocular depth estimation (cite NSFF, robust dynamic NeRF). Despite showing promising results in their papers, a reality check (cite dycheck) indicates that this is still challenging due to the following:
    \begin{itemize}
        \item Hand-crafted geometric and physics priors are limited, not sufficient to disambiguate motion and structure for in the wild data especially when the camera motion is smaller than the object motion. 
        \item Methods rely on monocular depth estimation tends to produce paper-thin foreground objects, and does not provide effective supervision for occluded regions.  These factors lead to severe artifacts when the dynamic object is close to the camera.
    \end{itemize}

\item We took inspiration from recent advance in text-to-3D generation, where 3D objects are generated by distillation from 2D text-to-image diffusion models. Our method is related to recent approaches which extend text-to-3D to image conditioned 3D generation, where researchers leverage various kinds of multi-view image diffusion models trained specifically for generating objects. Although effective for generating objects, we find these approaches are currently not directly applicable to our settings, because:
\begin{itemize}
        \item multi-view image diffusion models are currently trained for objects, not for general scenes with diverse foreground objects and complex background. \peiye{how does your 4D recon from monocular videos (i.e., a single-view case) link to multi-view diffusion? maybe add ``multi-novel-view supervision from mv diffusion priors" }
        \item domain gap between input real images and training set is significant, it is difficult to keep identity of the input scene when distill from pretrained text-to-image diffusion models.
        \item {\peiye{Should add the identity issue as well?}}
    \end{itemize}
\end{itemize}

Contributions:
We propose an effective method to leverage 2D diffusion priors \peiye{video diffusion cannot be categorized to 2D diffusion?} for reconstructing diverse dynamic scenes from casually captured monocular videos.
\begin{itemize}
    \item First we develop several strategies to help keep the identity of the target scene. By noticing that videos already include frames of the dynamic scene from various angles and time, we conveniently use the video frames to finetune 2D diffusion models (i.e. dreambooth) to learn the identity of the scene. To further reinforce the identity associated to each frames to reconstruct, we repurpose a pretrained video diffusion model to serve the function of an image-conditioned generation model.

    \item Applying dreambooth inevitably compromises the generalization ability of the image diffusion models, which leads to insufficient supervision for the novel views during training. To alleviate this issue, we propose to compensate the loss of generalizability with enhanced geometrical supervision using diffusion models that not only generate colors but depth map as well. 
    \item \peiye{Contributions can be better reorganized. Perhaps write this like: 1) for spatio-temporal consistency over frames, we use video sds, 2) for geometry consistency for every individual frame, we use RGB-D sds; 3) to reserve identity, we apply dreambooth; 4) ...}
\end{itemize}

\peiye{Taken together, we show how these holistic modifications address existing shortcomings and improve the quality of 4D recon}

Our method leads to .... state-of-the-art performance on the challenging dataset of dycheck.




% Method TODO:



% Experiment TODO:



% Ablation TODO:



% Paper TODO:

% Tables

% Method Figures

% Result Figures


